Biometrics: Trust, but Verify

Over the past two decades, biometric recognition has exploded into a plethora of different applications around the globe. This proliferation can be attributed to the high levels of authentication accuracy and user convenience that biometric recognition systems afford end-users. However, in-spite of the success of biometric recognition systems, there are a number of outstanding problems and concerns pertaining to the various sub-modules of biometric recognition systems that create an element of mistrust in their use - both by the scientific community and also the public at large. Some of these problems include: i) questions related to system recognition performance, ii) security (spoof attacks, adversarial attacks, template reconstruction attacks and demographic information leakage), iii) uncertainty over the bias and fairness of the systems to all users, iv) explainability of the seemingly black-box decisions made by most recognition systems, and v) concerns over data centralization and user privacy. In this paper, we provide an overview of each of the aforementioned open-ended challenges. We survey work that has been conducted to address each of these concerns and highlight the issues requiring further attention. Finally, we provide insights into how the biometric community can address core biometric recognition systems design issues to better instill trust, fairness, and security for all.

==> ch_overview.tex <==
\section{Biometrics: An Overview}

Prior to discussing the obstacles preventing trust in biometric recognition systems, it is useful to first give an overview of the state of biometric recognition systems. Doing so enables us to better understand the unique challenges researchers face in developing more trustworthy biometric recognition systems. To that end, we first provide a history of biometrics. Subsequently, we describe the inner workings of the biometric recognition pipeline. Finally, we give an overview of the different physical traits that have been utilized for biometric recognition systems.

\subsection{A Brief History of Biometrics}

\noindent \textbf{Ancient Biometrics: } The first known use of biometrics can be dated back to the Qin Dynasty (221-206 BC) where clay seals bearing friction ridge impressions from handprints were used as evidence during burglary investigations (see Figure~\ref{fig:history})~\cite{fingerprint_sourcebook}. This use-case of biometrics also showed up in sixteenth century China where inked palms and foot-soles were impressed on deeds of sale~\cite{fingerprint_sourcebook}. 

\vspace{5pt}
\noindent \textbf{Early Pioneers: } Years later in 1858, biometric recognition began to take hold in the west when a British colonial magistrate, William James Herschel, used fingerprints as a means of identifying people in Bengal, India~\cite{origin_fingerprinting}. Following the 1869 Habitual Criminals Act, in 1883, Alphonse Bertillon, devised a system to measure and record the dimensions of certain bony parts of the body (known as anthropometry or the Bertillon System)~\cite{bertillon}. These measurements were ``purportedly" unique to each individual and would not change over the course of their life. Bertillon also pioneered the concept of arrest photos (mugshots) taken simultaneously with bodily measurements and fingerprints.


The Bertillon System was generally accepted in many countries for the next three decades. However, the anthropometric measurement system took a serious hit in 1903, when a man named Will West was sentenced to the US Penitentiary at Leavenworth, Kansas. Upon further investigation, it was discovered there was already a prisoner at the penitentiary, named William West, whose Bertillon measurements were similar enough to identify both William and Will as the same person~\cite{william_west}. However, fingerprint comparisons quickly and correctly determined that William and Will were indeed two different people\footnote{According to prison records made public years later, the West men were apparently identical twins and each had a record of correspondence with the same immediate family relatives~\cite{history_fingerprints}}. As a consequence, Sir Edward Henry recommended adoption of fingerprinting as a replacement for the relatively indiscriminate Bertillon system. Scotland Yard adopted the Henry/Galton (Galton was a cousin of Charles Darwin, a polymath, and another pioneer of fingerprint recognition systems) fingerprint system in 1900~\cite{fingerprint_sourcebook}. For the first time, in 1905, fingerprints were successful in convicting a murderer in a British criminal case~\cite{british_crime}. Finally, in 1924, an act of congress established the Identification Division of the FBI~\cite{fbi_cjis}. Since then, the repository of fingerprints collected by the Identification Division has been indispensable in supporting American law enforcement. 

\vspace{5pt}
\noindent \textbf{Automation: } Following the early use-cases of biometrics in the forensics community which involved manual human comparisons, the first known research publication on automated biometric recognition was the one published by Mitchell Trauring in the journal~\emph{Nature} in 1963 on fingerprint matching~\cite{trauring1963automatic}. The development of automated biometric systems based on other traits such as voice~\cite{history_voice}, face~\cite{history_face}, and signature~\cite{history_signature} started in the 1960s. In 1972,~\emph{Identimat} was the first commercial-off-the-shelf (COTS) biometric recognition system~\cite{identimat}. 

\vspace{5pt}
\noindent \textbf{Government Adoption: } Following the success of \textit{automated} biometric recognition systems, government agencies began adoption. In July 1999, the FBI inaugurated the Integrated Automated Fingerprint Identification System (IAFIS), a large-scale fingerprint ID system for use in criminal investigations~\cite{iafis}. Following the aftermath of 9/11 terrorist attacks, the turn of the century witnessed a widespread adoption of biometric recognition for international border control. For instance, in 2003, the Department of Homeland Security (DHS) launched US-VISIT to authenticate international travelers via their fingerprints~\cite{us_visit}.

\vspace{5pt}
\noindent \textbf{Multi-Biometrics: } Beginning in 2008, the industry of automated biometric identification systems started moving beyond dependency on a single biometric trait (primarily fingerprints) to incorporating multiple additional biometric traits such as face and iris for improved accuracy and reliability. For instance, FBI Next Generation Identification (NGI) system was launched to expand IAFIS (primarily a fingerprint-based identification system) to include face and iris~\cite{fbi_ngi}. Across the globe in India, the Unique Identification Authority of India launched a project named Aadhar\footnote{Aadhar: a word meaning ``the foundation" in many Indian languages.} which currently serves as the world's largest multi-biometric database (fingerprint, face, and iris). Aadhaar is a voluntary program, with the goal of providing reliable national identification documents to most of India's estimated $1.36$ billion residents. Thus far, the Authority has enrolled more than $1.25$ billion Indian citizens based on their face, fingerprints, and irises~\cite{aadhar}. 

\vspace{5pt}
\noindent \textbf{Commercial Applications: } Aside from civil and criminal use-cases, the last decade has seen a boom in biometric recognition technology being widely adopted in commercial use. For example, in 2013, Apple launched ``TouchID", a fingerprint-based smartphone unlock system~\cite{touch_id}. Due to the user convenience and high recognition accuracy of ``TouchID", Apple Pay, an e-commerce application, has been widely adopted since 2014~\cite{apple_pay}. In 2017, Apple iPhones introduced ``FaceID", a touchless smartphone unlocking system via automated face recognition~\cite{face_id}. Finally, in 2020, Amazon introduced ``Amazon One"~\cite{amazon_one}, a contactless palmprint reader for conducting purchases at the Amazon Go stores.

All of these applications underscore that the accuracy and convenience of biometric recognition systems have come a long ways over centuries of study. It also demonstrates that a large proportion of the research in biometrics thus far has been aimed at system performance and adoption into applications. It is therefore not surprising that much of the work remaining towards developing trustworthy biometric recognition systems are related more towards questions of robustness, reliability, and security. In the following section, we examine from a more technical perspective, via an examination of the biometric pipeline, how modern day biometric recognition systems have become so accurate. At the same time, by laying out the inner workings of the biometric pipeline we set up a more systematic inspection of the remaining vulnerabilities and challenges that impede more trustworthy biometric recognition systems. 

\subsection{Biometric Recognition Pipeline}

A typical biometric recognition system has two stages of operation, namely, the enrollment stage and the recognition stage (see Figure~\ref{fig:pipeline}). In the enrollment stage, the biometric system acquires the biometric trait of an individual, extracts a salient feature set from it and stores the extracted feature set in a database (also referred to as a template), along with an identifier, label, and meta-data associating the feature set with an individual. During the recognition stage, the system once again acquires the biometric trait of an individual, extracts a feature set from it, and compares this feature set against the templates in the database with a matching algorithm in order to determine a match or to verify a claimed identity.

Biometric recognition systems are typically operated under two modes: (i) authentication (or verification) and (ii) search (or identification). If the objective is to~\emph{verify} the claimed identity of an individual, a query biometric sample needs to be compared only to an enrollment template corresponding to the claimed identity (one-to-one match). After comparing the two templates, we obtain a similarity measure (match score). If the match score is above a pre-defined threshold, then the identity claim is accepted. On the other hand, if the goal is to determine the user's identity without making any claims about who the user is, the query needs to be compared to the entire database of templates (one-to-many match). Typically, biometric recognition systems output two possible identification results: (i) one or more identities whose templates exhibit high similarity with the query biometric sample, or (ii) indicate that the query biometric sample has no associated templates enrolled in the gallery. If the biometric identification system is forced to output an identity, it is referred to as~\emph{closed-set} identification, whereas, the option to reject responses is known as~\emph{open-set} identification.

In both stages of enrollment and recognition and in both modes of authentication and search, the biometric recognition system utilizes a series of sub-modules. First, a biometric sensor (\eg, fingerprint reader or RGB camera) acquires the biometric trait (\eg, face, fingerprint, iris, voice, \etc) of a user in digital form. Subsequently, it is typical for a series of pre-processing steps to be applied to the raw digital output of the sensor. Next, the digitized trait is passed to a~\emph{feature extractor} to generate a compact and salient representation (or feature set) differentiating one user from another. This representation should have high \textit{inter-class variance}, \ie different users should have very different representations. In addition, the representation should have very low \textit{intra-class variance}, \ie two representations from the same user should be very similar. The representation could be based on handcrafted features (\eg fingerprint minutiae), deep features (\eg deep face representations), or a combination of handcrafted features with deep features (\eg through feature fusion). Finally, when a user needs to be authenticated or identified, a newly extracted representation can be compared to enrolled representation(s) with a matching algorithm.

At each stage (enrollment and recognition), mode (authentication and search), and sub-module (sensing, feature extraction, and matching) of the biometric recognition system, various vulnerabilities manifest themselves. In this paper, we highlight what these vulnerabilities are, and propose what can be done to address them in order to solidify more trust in biometric recognition systems. 



\subsection{Biometric Traits}
A final notable variable worth mentioning that impacts the specific vulnerabilities of a biometric recognition system is that of the choice of the physical trait being used (\ie different traits face different challenges and vulnerabilities). Indeed, a fundamental issue when designing any biometric system is the selection of the biometric trait. Ideally, any anatomical, behavioral, or physiological characteristic could be used as a biometric trait. However, in practice, biometric traits are limited by the following properties: (i) uniqueness, (ii) permanence, (iii) universality, (iv) collectability, (v) performance, (vi) user acceptance, and (vii) invulnerability~\cite{introduction_biometrics}. Thus far, every biometric trait has suffered in one of these seven properties leading to reduced trust in biometric systems in general. For example, face recognition systems are shown to perform better for certain demographics~\cite{howard2019effect, klare2012face, grother2019frvt} (a performance issue point (v)), fingerprint recognition often requires touching a sensor (not as hygienic as face image capture) (point (iv)), and both are vulnerable to a number of attacks (point (vii)). Since each trait may entail the use of different sensors, feature extractors, and matchers, each trait faces unique challenges. For example, deep network based face feature extractors have a vulnerability to adversarial attacks, while handcrafted minutiae features extracted from fingerprints may be more robust in this area.  

Due to the availability of large-scale legacy databases (\eg, driver's licence and immigration databases), and the closest satisfaction to points (i)-(vii) above, fingerprint and face recognition continue to be the most popular. While identifying people by their irises is being increasingly adopted for large-scale identification (\eg, the United Arab Emirates border crossing utilizes iris recognition), availability of legacy iris databases is limited. Finally, the National Institute of Standards and Technology (NIST) periodically benchmarks face~\cite{grother2019frvt}, fingerprint~\cite{nist_fpvte}, and iris~\cite{quinn2019irex} performance which has also contributed to the widespread adoption of these traits.

Aside from face, fingerprint, and iris, other biometric traits have also been proposed in literature, but are yet to attain sufficient level of technological maturity in points (i)-(vii) for deployment. Although this paper focuses on face and fingerprint due their widespread adoption, we note that other biometric traits, such as palmprint~\cite{palmprint}, voice~\cite{voice}, gait~\cite{gait}, signature~\cite{signature1, signature2}, hand geometry~\cite{hand_geomtery}, vascular patterns (palm vein~\cite{palm_vein}, hand vein~\cite{hand_vein}, or finger vein~\cite{finger_vein}), ear~\cite{ear}, retina/sclera~\cite{sclera}, keystroke dynamics~\cite{keystroke}, deoxyribonucleic acid (DNA)~\cite{dna}, electrocardiogram (ECG)~\cite{ecg}, and electroencephalogram (EEG)~\cite{eeg}, also suffer the five major points that reduces trust: (i) robustness to adverse noises, (ii) biasness, (iii) security from biometric attacks, (iv) explainability, and (v) privacy. 
